Region-Based Representations Revisited

We investigate whether region-based representations are effective for recognition. Regions were once a mainstay in recognition approaches, but pixel and patch-based features are now used almost exclusively. We show that recent class-agnostic segmenters like SAM can be effectively combined with strong unsupervised representations like DINOv2 and used for a wide variety of tasks, including semantic segmentation, object-based image retrieval, and multi-image analysis. Once the masks and features are extracted, these representations, even with linear decoders, enable competitive performance, making them well suited to applications that require custom queries. The compactness of the representation also makes it well-suited to video analysis and other problems requiring inference across many images.

==> sec/outline.tex <==
\section{Outline}
\subsection{Paper Structure}
\begin{enumerate}
    \item Section 1: Introduction 
    \begin{itemize}
        \item Earlier work used region representations for recognition and eventually was replaced by pixel-based CNNs and patch-based transformers 
        \item  Recent advances in foundation models like SAM and DINOv2 make it easier to use region-based representations 
        \item  We use region-based representations on per-pixel tasks as well as multi-image tasks where patch-based representations would be too big 
    \end{itemize}
    \item Section 2: Related Work
    \begin{itemize}
        \item Previous work on region-based representation including the paper `Unsupervised Discovery of Mid-level Discriminative Patches'. 
        \item Class-agnostic segmentation methods and SAM
        \item Dense feature representation learning and DINOv2 
        \item (If space?) Work related to the individual applications (semantic segmentation, video classification, 3D segmentation and object retrieval) 
    \end{itemize}
    \item Section 3: Method 
    \begin{itemize}
        \item Review key parts of SAM especially decoder and prompting 
        \item Process of combining DINOv2 with SAM (mean-pooling)
        \item Creating positional embeddings from DINOv2 
    \end{itemize}
    \item Section 4: Experiments (Semantic Segmentation)
    \begin{itemize}
        \item Sub-section on going from pixels to regions and back to pixels (region labeling) and SLIC) 
        \item Compare methods: DINOv2 with no SAM, DINOv2 SAM linear mean pooling, DINOv2 SAM linear max pooling, DINOv2 SAM MLP, DINOv2 SAM with SLIC. Datasets used: PASCAL-VOC, ADE20K
        \item Compare different feature representations: DINOv2, DINOv1, DenseCLIP, ImageNet pre-trained on Pascal-VOC, ADE20K
        \item Compare different SAM methods including the upper bound 
    \end{itemize}
    \item Section 5: Applications 
    \begin{itemize}
        \item Video Classification 
            \begin{itemize}
               \item Short explanation of how the method is used (more can be put into supplemental). Include that more frames can be used which could be useful for long videos 
                \item Experimental results  
            \end{itemize}
        \item 3D Segmentation 
        \begin{itemize}
               \item Short explanation of how method is used (more can be put into supplemental). Include that more images can be used at once to make predictions 
                \item Experimental results  
        \end{itemize}
        \item Object retrieval 
        \begin{itemize}
               \item Explain task and how it could be useful for active learning 
                \item Experimental results  
        \end{itemize}
    \end{itemize}
    \item Section 6: Conclusion
    \begin{itemize}
        \item Showed simple region based representation can be effective for pixel-based tasks as well as multi-image tasks
        \item List various areas of future work and other applications 
    \end{itemize}
     
\subsection{Contributions}
\begin{itemize}
    \item Simple region representation method using existing foundation models 
    \item Demonstrate how region representations have comparable performance on per-pixel tasks to patch-based representations 
    \item Demonstrate several applications where region representations can increase the amount of data (images) used  to train a model
\end{itemize}
\section{Figures and Tables}
\begin{itemize}
    \item Figures
    \begin{itemize} 
        \item Main method figure: includes SAM, DINO (could be called feature representation), mean pooling within DINO and averaging over DINO regions 
        \item Qualitative Results (Do not have have to use all of these)
        \begin{itemize}
            \item For video classification, can give an example of two closely related activities (such as exercising arm vs stretching arm and how including region information from frames is important 
            \item 3D segmentation results 
            \item Positional embedding illustrations 
        \end{itemize}
        \item Teaser figure: Could highlight the differences between pixel/patch-based representation and region-based representation 
    \end{itemize}
    \item Tables 
    \begin{itemize}
        \item Semantic Segmentation 
        \begin{itemize}
            \item  Method/Pooling Comparison: DINOv2 with no SAM, DINOv2 SAM linear mean pooling, DINOv2 SAM linear max pooling, DINOv2 SAM MLP, DINOv2 SAM with SLIC
            \item  Model Size: ViT-S, ViT-B, ViT-L, ViT-G 
            \item Dense Features: DINOv2, DINOv1, DenseCLIP, Image-Net pre-training 
            \item SAM region comparison: SAM, Mobile SAM, SAM HQ 
        \end{itemize}
       \item Video Classification for Kinetics-40
       \begin{itemize}
           \item DINOv2 avg pooling
           \item Our method 
       \end{itemize}
     \item 3D Segmentation
       \begin{itemize}
           \item DINOv2 avg pooling
           \item Our method 
       \end{itemize}
       \item Object Retrieval. On COCO and if time LVIS 
       \begin{itemize}
           \item CLIP (image-level): Cosine similarity between CLIP image features of image and CLIP image features of query object 
           \item DINOv2 (image-level): Same as above except with DINOv2
           \item Our method   
       \end{itemize}
        
    \end{itemize}
    \item 
\end{itemize}

\end{enumerate}

==> tables/compare_pe_slic.tex <==
\begin{table}[]
    \centering
    \small 
    \caption{\textbf{Comparison of positional embedding and SLIC }}
    \begin{tabular}{lcc}
        \toprule
        Region or Patch& Pascal VOC & ADE20K \\ 
        \midrule
        PE &   83.7& 50.6\\
        SAM and SLIC & 86.8 & 52.8 \\
        PE, SAM and SLIC  & 86.9  & 52.9 \\
        \bottomrule
    \end{tabular}
    \label{tab:pe_slic}
\end{table}

==> tables/scannet_training_param.tex <==
\begin{table*}[]
    \centering
    \caption{\textbf{Scene-Level Semantic Segmentation Training Hyper-Parameters}}
    \begin{tabular}{lcccccc}
        \toprule
         \multirow{2}{*}{Architecture}  & \multicolumn{2}{c}{Initial LR} & \multicolumn{2}{c}{Batch Size} & \multicolumn{2}{c}{Epochs}\\ 
         & Pascal-VOC & ADE20K & Pascal-VOC & ADE20K & Pascal-VOC &ADE20K\\
        \midrule
        Linear (Regions) & 5e-4&5e-4&32 regions&8192 regions &20 &100\\  
        Linear (Patch) & 1e-3&1e-3&8 images&16 images&20&20\\
        MLP (hidden size: 1000) & 5e-4 & 1e-4 & 32 regions & 8192 regions & 4&28  \\       
        Transformer & 1e-4 & 1e-4 & 2 images & 2 images&4&8\\   
        \bottomrule
    
    \end{tabular}
    \label{tab:scannet_training_param}

\end{table*}

==> tables/slic_sem_seg.tex <==
\begin{table}[]
    \centering
    \small 
    \caption{\textbf{Semantic segmentation via region classification.}  All methods use a linear probe on frozen DINOv2 features. Models are evaluated on validation sets, with $^*$ indicating numbers reported in the original paper. The DINOv2 baseline does not propose regions, but directly predicts pixel classes on the upsampled image features. \ansel{I moved the SAM variants + SLIC into an ablations table at the end, as this table can emphasize that ``incorporating regions into features improves semantic segmentation.''}}
    \begin{tabular}{lcc}
        \toprule
        & Pascal VOC & ADE20K \\ 
        \midrule
        DINOv2 \cite{dinov2}& & \;\,47.7$^*$ \\
        SAM \cite{SAM} &  81.9 & 50.2 \\
        SAM + SLIC & \textbf{88.3} & \textbf{52.8} \\
        \bottomrule
    \end{tabular}

    \label{tab:ss_region_gen}
\end{table}

==> tables/video_classification.tex <==
\begin{table}[h]
\caption{
    \textbf{Activity recognition with regions on Kinetic 400~\cite{kay2017kinetics}}. We take the linear probe result from DINOv2's paper~\cite{oquab2023dinov2}, which reports the best result in a 102-trial hyperparameter sweep. They find that averaging the CLS tokens outperforms concatenation. %Using patch features with a transformer is not viable due to their large quantity.
}
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccc}
\toprule
{Model} & {Input} & {Accuracy $\uparrow$} \\
\midrule
Linear Probe & Average CLS tokens & 76.3 \\
%Transformer & Patch features & - \\
Transformer &  Region features & 79.5 \\

\bottomrule
\end{tabular}
}
\label{tab:video_classification}
\vspace{-3pt}
\end{table}


